Particle yields from numerical simulations

In this paper we use numerical simulations to calculate the particle yields. We demonstrate that in the model of local particle creation the deviation from the pure exponential distribution is natural even in equilibrium, and an approximate Tsallis-Pareto-like distribution function can be well fitted to the calculated yields, in accordance with the experimental observations. We present numerical simulations in classical $\Phi^4$ model as well as in the SU(3) quantum Yang-Mills theory to clarify this issue.

==> endistrCleymans.tex <==
\begin{figure}[h!t]
\centering
\includegraphics[width=0.55\linewidth]{./Kepek/fig2_cleymans_worku_iop.png}
\caption{Transverse momentum distribution for $K^0_S$ as measured by the CMS collaboration \cite{Khachatryan:2011tm}. The \mbox{$0.9$ TeV} data is compared to the Tsallis-B distribution (continuous full line) by J. Cleymans and D. Worku in \cite{Cleymans:2011in}. }
\label{fig:endistrCleymans}
\end{figure}

==> multifit.tex <==
\begin{figure}[!ht] 
\centering
 \subfloat
 { \begin{overpic}[scale=0.55]{./Kepek/MultiFit_1x5_17.pdf}
 	\put (-3,15){\rotatebox{90}{{\footnotesize Num. of data (log)}}}
    \put (41,-3){{\footnotesize Energy-density}
    \put (-30,-9){{\small {\color{blue}(a)} uniform init.}}}
 \end{overpic}}
 \subfloat
 {\begin{overpic}[scale=0.55]{./Kepek/MultiFit_1x5LorMod_17.pdf}
 	 %	\put (-2,5){\rotatebox{90}{\tiny{ Num. of data (log)}}}
    \put (41,-3){{\footnotesize Energy-density}
    \put (-25,-9){{\footnotesize {\color{blue}(b)} sech init.}}}
 \end{overpic}}
\vspace{18 pt}
   \caption{{Various fits on logscale energy histogram}}
  \label{fig:multifit}
\end{figure}
